Optimal Vertex-Cut Sparsification of Quasi-Bipartite Graphs

In vertex-cut sparsification, given a graph $G=(V,E)$ with a terminal set $T\subseteq V$, we wish to construct a graph $G'=(V',E')$ with $T\subseteq V'$, such that for every two sets of terminals $A,B\subseteq T$, the size of a minimum $(A,B)$-vertex-cut in $G'$ is the same as in $G$. In the most basic setting, $G$ is unweighted and undirected, and we wish to bound the size of $G'$ by a function of $k=|T|$. Kratsch and Wahlstr\"om [JACM 2020] proved that every graph $G$ (possibly directed), admits a vertex-cut sparsifier $G'$ with $O(k^3)$ vertices, which can in fact be constructed in randomized polynomial time. We study (possibly directed) graphs $G$ that are quasi-bipartite, i.e., every edge has at least one endpoint in $T$, and prove that they admit a vertex-cut sparsifier with $O(k^2)$ edges and vertices, which can in fact be constructed in deterministic polynomial time. In fact, this bound naturally extends to all graphs with a small separator into bounded-size sets. Finally, we prove information-theoretically a nearly-matching lower bound, i.e., that $\tilde{\Omega}(k^2)$ edges are required to sparsify quasi-bipartite undirected graphs.

==> SparseConstruction.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,445); %set diagram left start at 0, and has height of 445

%Rounded Rect [id:dp19626210799558663] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=2.25]  (311,86.93) .. controls (311,79.97) and (316.64,74.33) .. (323.6,74.33) -- (361.4,74.33) .. controls (368.36,74.33) and (374,79.97) .. (374,86.93) -- (374,420.73) .. controls (374,427.69) and (368.36,433.33) .. (361.4,433.33) -- (323.6,433.33) .. controls (316.64,433.33) and (311,427.69) .. (311,420.73) -- cycle ;
%Rounded Rect [id:dp4452386118793552] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  (433,68.33) .. controls (433,61.82) and (438.28,56.53) .. (444.8,56.53) -- (480.2,56.53) .. controls (486.72,56.53) and (492,61.82) .. (492,68.33) -- (492,309.53) .. controls (492,316.05) and (486.72,321.33) .. (480.2,321.33) -- (444.8,321.33) .. controls (438.28,321.33) and (433,316.05) .. (433,309.53) -- cycle ;
%Shape: Circle [id:dp8209252493475421] 
\draw   (194,83.5) .. controls (194,72.18) and (203.18,63) .. (214.5,63) .. controls (225.82,63) and (235,72.18) .. (235,83.5) .. controls (235,94.82) and (225.82,104) .. (214.5,104) .. controls (203.18,104) and (194,94.82) .. (194,83.5) -- cycle ;
%Shape: Circle [id:dp3311599247988861] 
\draw   (320,33.5) .. controls (320,22.18) and (329.18,13) .. (340.5,13) .. controls (351.82,13) and (361,22.18) .. (361,33.5) .. controls (361,44.82) and (351.82,54) .. (340.5,54) .. controls (329.18,54) and (320,44.82) .. (320,33.5) -- cycle ;
%Straight Lines [id:da24881520323803286] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (232,71) -- (315.12,40.69) ;
\draw [shift={(317,40)}, rotate = 159.96] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp4815136078729607] 
\draw   (441,82.5) .. controls (441,71.18) and (450.18,62) .. (461.5,62) .. controls (472.82,62) and (482,71.18) .. (482,82.5) .. controls (482,93.82) and (472.82,103) .. (461.5,103) .. controls (450.18,103) and (441,93.82) .. (441,82.5) -- cycle ;
%Straight Lines [id:da9050420984976184] 
\draw    (362,41) -- (440.14,72.26) ;
\draw [shift={(442,73)}, rotate = 201.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp9161011210155758] 
\draw   (321,107.5) .. controls (321,96.18) and (330.18,87) .. (341.5,87) .. controls (352.82,87) and (362,96.18) .. (362,107.5) .. controls (362,118.82) and (352.82,128) .. (341.5,128) .. controls (330.18,128) and (321,118.82) .. (321,107.5) -- cycle ;
%Straight Lines [id:da020527886673509466] 
\draw    (234,92) -- (317.07,114.48) ;
\draw [shift={(319,115)}, rotate = 195.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da21967763076410418] 
\draw    (362,114) -- (438.08,92.54) ;
\draw [shift={(440,92)}, rotate = 164.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp033720785202185466] 
\draw   (322,208.5) .. controls (322,197.18) and (331.18,188) .. (342.5,188) .. controls (353.82,188) and (363,197.18) .. (363,208.5) .. controls (363,219.82) and (353.82,229) .. (342.5,229) .. controls (331.18,229) and (322,219.82) .. (322,208.5) -- cycle ;
%Straight Lines [id:da43134112973399974] 
\draw    (228,100.33) -- (320.69,206.99) ;
\draw [shift={(322,208.5)}, rotate = 229.01] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp8887161263051901] 
\draw   (198,247.5) .. controls (198,236.18) and (207.18,227) .. (218.5,227) .. controls (229.82,227) and (239,236.18) .. (239,247.5) .. controls (239,258.82) and (229.82,268) .. (218.5,268) .. controls (207.18,268) and (198,258.82) .. (198,247.5) -- cycle ;
%Straight Lines [id:da6207049921554524] 
\draw    (237,236) -- (319.07,214.51) ;
\draw [shift={(321,214)}, rotate = 165.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp726453929749838] 
\draw   (445,346.5) .. controls (445,335.18) and (454.18,326) .. (465.5,326) .. controls (476.82,326) and (486,335.18) .. (486,346.5) .. controls (486,357.82) and (476.82,367) .. (465.5,367) .. controls (454.18,367) and (445,357.82) .. (445,346.5) -- cycle ;
%Shape: Circle [id:dp06351426052177844] 
\draw   (443,208.5) .. controls (443,197.18) and (452.18,188) .. (463.5,188) .. controls (474.82,188) and (484,197.18) .. (484,208.5) .. controls (484,219.82) and (474.82,229) .. (463.5,229) .. controls (452.18,229) and (443,219.82) .. (443,208.5) -- cycle ;
%Straight Lines [id:da5206561596955621] 
\draw    (363,208.5) -- (441,208.5) ;
\draw [shift={(443,208.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3603326415371011] 
\draw    (356,226.33) -- (443.78,340.91) ;
\draw [shift={(445,342.5)}, rotate = 232.54] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp6653954310477737] 
\draw   (444,295.5) .. controls (444,284.18) and (453.18,275) .. (464.5,275) .. controls (475.82,275) and (485,284.18) .. (485,295.5) .. controls (485,306.82) and (475.82,316) .. (464.5,316) .. controls (453.18,316) and (444,306.82) .. (444,295.5) -- cycle ;
%Rounded Rect [id:dp8045724964210699] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=2.25]  (313,333.33) .. controls (313,326.82) and (318.28,321.53) .. (324.8,321.53) -- (360.2,321.53) .. controls (366.72,321.53) and (372,326.82) .. (372,333.33) -- (372,418.53) .. controls (372,425.05) and (366.72,430.33) .. (360.2,430.33) -- (324.8,430.33) .. controls (318.28,430.33) and (313,425.05) .. (313,418.53) -- cycle ;
%Shape: Circle [id:dp7609470110835062] 
\draw   (319,295.5) .. controls (319,284.18) and (328.18,275) .. (339.5,275) .. controls (350.82,275) and (360,284.18) .. (360,295.5) .. controls (360,306.82) and (350.82,316) .. (339.5,316) .. controls (328.18,316) and (319,306.82) .. (319,295.5) -- cycle ;
%Straight Lines [id:da7633429739186921] 
\draw    (360,295.5) -- (438,295.5) ;
\draw [shift={(440,295.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da11081577871365234] 
\draw    (223,103) -- (321.03,278.59) ;
\draw [shift={(322,280.33)}, rotate = 240.83] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Circle [id:dp5417874641949081] 
\draw   (320,348.5) .. controls (320,337.18) and (329.18,328) .. (340.5,328) .. controls (351.82,328) and (361,337.18) .. (361,348.5) .. controls (361,359.82) and (351.82,369) .. (340.5,369) .. controls (329.18,369) and (320,359.82) .. (320,348.5) -- cycle ;
%Straight Lines [id:da3843793440130767] 
\draw    (214.5,104) -- (321.15,332.19) ;
\draw [shift={(322,334)}, rotate = 244.95] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da18745014688869088] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (486,346.5) .. controls (558.27,319.77) and (561.93,240.11) .. (486.32,209.42) ;
\draw [shift={(484,208.5)}, rotate = 21.04] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;
%Straight Lines [id:da7037929918641701] 
\draw    (361,348.5) -- (439,348.5) ;
\draw [shift={(441,348.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da0199002801842334] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (342.5,133) -- (342.5,183) ;
%Straight Lines [id:da31588609058397554] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (342.5,239) -- (342.5,268) ;
%Straight Lines [id:da3800798037019355] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (461.5,111) -- (461.5,175) ;
%Straight Lines [id:da7553573904397404] 
\draw [line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (463.5,238) -- (463.5,269) ;
%Curve Lines [id:da6253180992393452] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (362,114) .. controls (387.48,84.6) and (389.91,80.17) .. (363.64,43.3) ;
\draw [shift={(362,41)}, rotate = 54.32] [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

% Text Node
\draw (208,81) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle a$};
% Text Node
\draw (333,23) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle v_{0} \ $};
% Text Node
\draw (453,73) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle b_{1}$};
% Text Node
\draw (236,28) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{0} \ \notin E'$};
% Text Node
\draw (334,97) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle v_{1} \ $};
% Text Node
\draw (335,198) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle v_{j} \ $};
% Text Node
\draw (212,237) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle a'$};
% Text Node
\draw (457,337) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle b_{i}$};
% Text Node
\draw (455,197) node [anchor=north west][inner sep=0.75pt]  [font=\large] [align=left] {$\displaystyle b_{j}$};
% Text Node
\draw (289,154) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{j}$};
% Text Node
\draw (276,82) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{1}$};
% Text Node
\draw (453,287) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {$\displaystyle b_{i-1}$};
% Text Node
\draw (331,291) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {$\displaystyle v_{i-1} \ $};
% Text Node
\draw (276.25,184.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{i-1}$};
% Text Node
\draw (335,348) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {$\displaystyle v_{i} \ $};
% Text Node
\draw (288,247) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{i}$};
% Text Node
\draw (544,265) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {$\displaystyle f$};


\end{tikzpicture}

